Decomposable Submodular Function Minimization via Maximum Flow

This paper bridges discrete and continuous optimization approaches for decomposable submodular function minimization, in both the standard and parametric settings. We provide improved running times for this problem by reducing it to a number of calls to a maximum flow oracle. When each function in the decomposition acts on $O(1)$ elements of the ground set $V$ and is polynomially bounded, our running time is up to polylogarithmic factors equal to that of solving maximum flow in a sparse graph with $O(\vert V \vert)$ vertices and polynomial integral capacities. We achieve this by providing a simple iterative method which can optimize to high precision any convex function defined on the submodular base polytope, provided we can efficiently minimize it on the base polytope corresponding to the cut function of a certain graph that we construct. We solve this minimization problem by lifting the solutions of a parametric cut problem, which we obtain via a new efficient combinatorial reduction to maximum flow. This reduction is of independent interest and implies some previously unknown bounds for the parametric minimum $s,t$-cut problem in multiple settings.

==> assumption.tex <==

\section{Removing  Assumptions on $F_i$}\label{sec:assumptions}
In this section we argue why the assumptions on the functions $F_i$ introduced in Section~\ref{sec:prelim} are valid without loss of generality. More precisely, we assumed that for all $i$, $F_i(\emptyset) = F_i(V_i) = 0$ and $F_i(S) \geq 0$ for all $S$.
Here we show that a simple preprocessing step can enforce all of these conditions.

Without changing the original problem we can shift each $F_i$ such that it evaluates to $0$ on $\emptyset$, by defining ${\overline{F}}_i(S) = F_i(S) - F_i(\emptyset)$. This only changes $F$ by a constant term without affecting the sets that minimize the parametric problem  (\ref{eq:parametric-def}).

For each $i$, we use Lemma~\ref{lem:opt-base-poly} to find a point $w_i \in B(\overline{F}_i)$. Using this point, we define $\overline{\overline{F}}_i(S) = \overline{F}_i(S) - w_i(S)$. Since by definition $w_i(V_i) = \overline{F}_i(V_i)$, we have that $\overline{\overline{F}}_i(V_i) = 0$. Also, we have $\overline{\overline{F}}_i(\emptyset) = \overline{F}_i(\emptyset)  = 0$. Finally, since $w_i(S) \leq \overline{F}_i(S)$ for all $S$, we also have $\overline{\overline{F}}_i(S) \geq 0$.


Now we can equivalently rewrite the parametric problem
\begin{align*}
F_\alpha(A) &= F(A) + \sum_{j \in A}   \psi_j'(\alpha) \\
&= \overline{F}(A) + \sum_{j \in A}   \psi_j'(\alpha) + \left( \sum_{i=1}^m F_i(\emptyset) \right) \\
&= \overline{\overline{F}}(A) + \sum_{j \in A} \left(  \psi_j'(\alpha) + \sum_{i=1}^\m w_i(j) \right) + \left( \sum_{i=1}^m F_i(\emptyset) \right)\,. \\
\end{align*}
Now we can solve the problem on $\overline{\overline{F}} = \sum_{i=1}^{\m} \overline{\overline{F}}_i$ with the parametric penalties $\overline{\overline{\psi}}'_j (\alpha) = \psi'_j(\alpha) + \sum_{i=1}^\m w_i(j)$, which maintain the validity of Assumption~\ref{defn:conditions}.

To compute a point in the base polytope of a submodular function we use the following folklore lemma, which shows that the running time of our initialization procedure is $O(\sum_{i=1}^\m \vert V_i \vert \cdot \evo_i)$:
\begin{lem}\label{lem:opt-base-poly}
Let $F : 2^V \rightarrow \mathbb{Z}$ be a submodular set function, with $F(\emptyset) = 0$, and let $B(F)$ be its base polytope. Given any $x \in \mathbb{R}^{\vert V \vert}$, one can compute
\[
\arg\max_{w \in B(F)} \langle x, w\rangle
\]
 using $O(\vert V \vert)$ calls to an evaluation oracle for $F$. Furthermore $w$ is integral.
\end{lem}

